Towards Trustworthy LLMs for Code: A Data-Centric Synergistic Auditing Framework

LLM-powered coding and development assistants have become prevalent to programmers' workflows. However, concerns about the trustworthiness of LLMs for code persist despite their widespread use. Much of the existing research focused on either training or evaluation, raising questions about whether stakeholders in training and evaluation align in their understanding of model trustworthiness and whether they can move toward a unified direction. In this paper, we propose a vision for a unified trustworthiness auditing framework, DataTrust, which adopts a data-centric approach that synergistically emphasizes both training and evaluation data and their correlations. DataTrust aims to connect model trustworthiness indicators in evaluation with data quality indicators in training. It autonomously inspects training data and evaluates model trustworthiness using synthesized data, attributing potential causes from specific evaluation data to corresponding training data and refining indicator connections. Additionally, a trustworthiness arena powered by DataTrust will engage crowdsourced input and deliver quantitative outcomes. We outline the benefits that various stakeholders can gain from DataTrust and discuss the challenges and opportunities it presents.

==> sections/roadmap.tex <==
\section{Road Ahead}

We explore the challenges and opportunities associated with realizing the vision of \tool.
% and offer trustworthiness-related recommendations for both LLM developers and users.

% \subsection{Challenges and Opportunities in Trustworthiness Auditing}
\textbf{Tools Integration in Training Data Inspection.} Existing scanning tools come with different prerequisites and input/output formats, often offering a variety of configuration options to support diverse scanning scenarios. For example, when using Infer~\cite{infer} to detect software defects and vulnerabilities, the input must be a compilable code project, and numerous options can be customized to meet specific detection needs. This complexity makes it challenging to integrate various scanning tools effectively, but it also presents opportunities for future research and innovation. First, designing unified input/output formats or domain-specific languages (DSLs) for tool integration can greatly enhance the extensibility of training data inspections. Second, utilizing on-demand configuration selection through agents can significantly improve the flexibility and efficiency of inspections, enabling more targeted and customizable analyses. Third, aggregating the results from different scanning or analysis tools can lead to more confident and reliable inspection decisions, increasing the overall trustworthiness of the process.

\textbf{Resources Aggregation in Evaluation Data Synthesis.} Similar to the scanning tools used in training data inspection, the crowd resources in evaluation data synthesis are often heterogeneous and written in informal free text (\eg Stack Overflow posts). This presents similar challenges in integrating these diverse resources, while also offering research opportunities. For instance, designing DSLs for consistent information representation, developing automatic and adaptive data crawling and parsing methods, and conducting information fusion and conflict resolution are promising areas of exploration. The latter two directions may require leveraging the capabilities of LLMs or LLM-based agents for tasks such as website exploration, code generation (\eg scripts for HTML parsing), and information understanding and summarization.

\textbf{Methods Adoption in Root Cause Attribution.} Although existing instance-level attribution methods, such as influence functions and gradient-based analysis, have shown promising effectiveness in certain domains and data modalities~\cite{}, their performance in code-related data analysis remains underexplored and unvalidated. This presents potential risks in applying these methods to root cause attribution in the context of LLMs for code. However, it also suggests opportunities for in-depth analysis of these methods, potentially leading to code-specific adaptations that enhance their effectiveness in this domain. In addition, developing effective approaches for combining the analysis results of instance-level methods and guiding pattern-level attribution (\ie incremental training data inspection) remains a challenge that requires further exploration. For example, a dedicated mechanism should be designed to ensure the accuracy of common patterns extracted from issues identified through evaluation data, which can then be used to guide pattern-level attribution.


\textbf{Interaction Paradigm in Trustworthiness Arena.} Unlike the Chatbot Arena, where task formats (\eg chatting with LLMs) are usually straightforward for general users, our trustworthiness arena faces a higher participation threshold due to the complexity and specialized nature of certain trustworthiness dimensions. For example, in code security assessments, even many experienced developers may struggle to effectively identify or verify software vulnerabilities in code. This challenge necessitates designing more participatory interaction and task paradigms by simplifying or reorganizing the problem. For instance, we can generate a checklist of fine-grained, low-level safeguard operations (\eg index range validation) for potentially vulnerable code and ask users to verify it.


% \subsection{Recommendations for Code LLM Developers and Users}
